Precision Profile Pollution Attack on Sequential Recommenders via Influence Function

Sequential recommendation approaches have demonstrated remarkable proficiency in modeling user preferences. Nevertheless, they are susceptible to profile pollution attacks (PPA), wherein items are introduced into a user's interaction history deliberately to influence the recommendation list. Since retraining the model for each polluted item is time-consuming, recent PPAs estimate item influence based on gradient directions to identify the most effective attack candidates. However, the actual item representations diverge significantly from the gradients, resulting in disparate outcomes.To tackle this challenge, we introduce an INFluence Function-based Attack approach INFAttack that offers a more accurate estimation of the influence of polluting items. Specifically, we calculate the modifications to the original model using the influence function when generating polluted sequences by introducing specific items. Subsequently, we choose the sequence that has been most significantly influenced to substitute the original sequence, thus promoting the target item. Comprehensive experiments conducted on five real-world datasets illustrate that INFAttack surpasses all baseline methods and consistently delivers stable attack performance for both popular and unpopular items.

==> 3_problem-method_backup.tex <==
\section{Problem Formulation}

\textbf{Sequential Recommendation}. We denote a sequential recommender model by $f_\theta$, where $\theta$ represents the learnable parameters of the model. Let $u\in \mathcal{U}$ and $v\in \mathcal{V}$ denote a user and an item, respectively, where $\mathcal{U}$ ($\mathcal{V}$) denotes the set of all users (items). We assume there are $n$ users and $m$ items, \textit{i.e.}, $|\mathcal{U}|=n$ and $|\mathcal{V}|=m$, and each user associates with a chronological sequence $\bm{x}_{u}=[v_1,\dots,v_t,\dots,v_{T}]$, where $v_{t}$ denotes the $t$-th interacted item by $u$. Let $\mathcal{X}=\{\bm{x}_{u}|u\in\mathcal{U}\}$ denote the interaction sequences of all user. Then, the model parameters of the recommender model $f_\theta$ are learned by fitting $\mathcal{X}$. Formally, the learning objective is defined as
\begin{equation} \label{eq:training-loss}
    \hat{\theta} = argmin_{\theta} \frac{1}{n} \sum_{u\in\mathcal{U}} L(\bm{x}_{u};\theta),
\end{equation}
where $L(\bm{x}_{u},\theta)$ is the loss for fitting $u$'s sequence $\bm{x}_{u}$, which can be varied due to the choice of training strategy of the sequential model\footnote{For example, it could be different for SASRec~\cite{DBLP:conf/icdm/KangM18} and Bert4Rec~\cite{DBLP:conf/cikm/SunLWPLOJ19}. Specifically, we use the loss taken by the paper proposing the recommender model.}. During testing, the learned model $f_{\hat{\theta}}$ could generate a recommendation score for each candidate item, indicating how likely the item would be the $(T\text{+}1)$-th interacted item. The final recommendation list is generated based on the scores.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/attack-goal.png}
    \caption{Profile pollution attack problem defined in this work for sequential recommendation:  an attacker injects certain items into a user's interaction sequence to create polluted sequences, such that the model trained on the polluted data could enhance the recommendation of a target item compared to the model trained on the clearing data.}
     \vspace{-2mm}
    \label{fig:attack-flow}
    \vspace{-2mm}
\end{figure}

\vspace{+5pt}
\noindent \textbf{Profile Pollution Attack}. In this work, as shown in Figure~\ref{fig:attack-flow}, we consider the scenario where an attacker can inject certain items into the training sequences of users to perform a profile pollution attack in sequential recommendation, aiming at boosting the recommendation of a target item. Specifically, similar to previous work~\cite{DBLP:conf/recsys/YueZKSW22}, we make the following assumptions to define our research scope:

\begin{itemize}[leftmargin=*]
\item \textbf{Data Access and Manipulation}: The attacker has access to the original training data $\mathcal{X}$ and item set $\mathcal{V}$. For each training sequence $\bm{x}_{u}=[v_{1},\dots,v_{T}] \in \mathcal{X}$, the attacker can insert $K$ items $[v_{1}^{\prime},\dots, v_{K}^{\prime}]$ (\eg via malware~\cite{DBLP:conf/kbse/LeeHR17}) to construct an attacked sequence $\bm{x}_{u}^{\prime} = [v_1,\dots,v_{T},v_{1}^{\prime},\dots, v_{L}^{\prime}]$. This results in an attacked dataset $\mathcal{X}^{\prime} = \{\bm{x}_{u}^{\prime}|u\in\mathcal{U}\}$.
\item \textbf{White-box Attacks}: The attacker knows the sequential model $f_\theta$, as well as the training loss in Equation~\eqref{eq:training-loss}.

\item \textbf{Limited Insertion}: The amount of injected items $K$ is controlled to ensure that the recommendation system can maintain good performance after the attack.

\item \textbf{Attack without Delay}: The attacker can finish manipulating the training data before the recommender system starts training. Therefore, the sequential model parameters of $f_{\theta}$ will indeed be learned by fitting $\mathcal{X}^{\prime}$, \ie
$$\hat{\theta}^{\prime} = \arg\min_{\theta} \sum_{u\in\mathcal{U}} L(\bm{x}_{u}^{\prime};\theta),$$
where $\hat{\theta}^{\prime}$ denotes the learned model parameters based on $\mathcal{X}^{\prime}$, and $L(\cdot)$ is the same function used in Equation~\eqref{eq:training-loss}. 

\end{itemize}

\textit{Attack goal}: our attack goal is to find a $\mathcal{X}^{\prime}$ such that $f_{\hat{\theta}^{\prime}}$ can boost the recommendation of a target item $v^{*} \in \mathcal{V}$ as much as possible\footnote{Indeed, the attacker can also downgrade the recommendation of a target item. The goal can be achieved by promoting other items, so we only focus on promoting the target items in this work.}, compared to $f_{\hat{\theta}}$ trained with the original training data $\mathcal{X}$.



\section{Attack Plan Based on Influence Function}
In this section, we introduce the proposed attack algorithm. Firstly, we present the overall framework and then elaborate on the main components. Lastly, we provide a detailed algorithm.

\subsection{Overview}
To achieve our attack goal in the sequential recommendation, we propose an  \textit{\textbf{INF}luence function-based \textbf{Attack} } (INFAttack)  framework, which includes two main steps as shown in Figure~\ref{fig:attack-model}:
\begin{itemize}[leftmargin=*]

   \item Step 1: Candidate polluted sequence generation (the left box of Figure~\ref{fig:attack-model}). We first enumerate all possible combinations of injected items into one item, generating $m$ ($m=|\mathcal{V}|$) possible combinations. Then, for each original sequence $\bm{x}{u} \in \mathcal{X}$, we inject every possible combination into $\bm{x}{u}$, forming m contaminations sequence. Then, by filtering the pollution sequence, the optimal pollution sequence is obtained as the initial pollution sequence, and this step is repeated K times to obtain the final pollution sequence.
    
     % \item Step 1: Candidate polluted sequence generation (the left box of Figure~\ref{fig:attack-model}).  We first enumerate all possible combinations of the $K$ injected items, generating $m$ ($m=|\mathcal{V}|$) possible combinations. Then, for each original sequence $\bm{x}_{u} \in \mathcal{X}$, we inject each possible combination into $\bm{x}_{u}$, forming all possible polluted sequences for it. 
     
    
    \item Step 2: Polluted sequence screening. The objective of this step is to select appropriate pollution sequences for users, thereby constructing the attacked dataset $\mathcal{X}^{\prime}$ and ensuring the efficacy of the attack. However, directly identifying the optimal combination of pollution sequences for all users proves arduous as a result of the vast selection space of $m*n$ ($n=|\mathcal{U}|$). Therefore, we adopt a greedy approach~\cite{DBLP:conf/kdd/ZugnerAG18} to execute this phase, which entails selecting the most influential pollution sequence for each user in terms of boosting the target item, instead of immediately determining the best composition of pollution sequences across all users. The resultant individual pollution sequences are then integrated into $\mathcal{X}^{\prime}$. The influential impact on the target item is gauged using the influence function~\cite{DBLP:conf/icml/KohL17}. The right box of Figure~\ref{fig:attack-model} shows the process.
\end{itemize}



In summary, our approach entails an exhaustive enumeration of all feasible polluted sequences, followed by a meticulous selection process using a greedy approach based on the influence function to prioritize the most influential ones for enhancing the recommendation of the target item, culminating in the creation of the final attacked dataset. Unlike gradient-based methods that experience diminished attack efficacy during the conversion of gradient-based attacks into real-world item sequences~\cite{DBLP:conf/recsys/YueHZM21, DBLP:conf/recsys/YueZKSW22}, INFAttack directly manipulates genuine items to generate polluted sequences, thereby ensuring optimal attack effectiveness for actual item sequences\footnote{At a local level.}. We next elaborate on the two main steps.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]
    {img/attack-model-acr.png}
    \caption{ The overall framework of the proposed INFAttack method, which mainly includes two parts: 1) candidate polluted sequence generation; and 2) polluted sequence screening.}
     \vspace{-2mm}
    \label{fig:attack-model}
    \vspace{-2mm}
\end{figure}



\subsection{Candidate Polluted Sequence Generation}
As previously mentioned, we inject $K$ items to construct a polluted sequence. To generate all possible candidate polluted sequences, we first enumerated all possible combinations of $[v_{1}^{\prime},\dots,v_{K}^{\prime}]$ (\ie the $K$ injected items) from the item set $\mathcal{V}$, generating $m$ ($m=|\mathcal{V}|$) possible combinations. Then, for a original sequence $\bm{x}_{u} \in \mathcal{X}$, we inject each possible $[v_{1}^{\prime},\dots,v_{K}^{\prime}]$ into $\bm{x}_{u}$, getting the polluted sequence $\bm{x}_{u(\delta)}=[v_{1},\dots,v_{T},v_{1}^{\prime},\dots,v_{K}^{\prime}]$. Finally, for each $\bm{x}_{u}$, this process results in the candidate set of polluted sequences, denoted as $\{\bm{x}_{u(\delta_{p})}|p=1,\dots,m\}$ for user $u$, where $\bm{x}_{u(\delta_{p})}$ denotes the $p$-th possible polluted sequence. As shown in Figure~\ref{fig:method-Tvalue}, for each $\bm{x}_{u}$, there are $m$ possible candidate polluted sequences when $K=1$. By calculating the optimal sequence when k=1, repeat the process to calculate $K=2$. There are $m$ possible candidate polluted sequences when $K=2$.  




\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/method-Tvalue.png}
    \caption{Illustration of generating candidate polluted sequences: (a) the case of injecting $1$ item, resulting in $m$ candidate polluted sequences; (b) the case of injecting $2$ items, resulting in $m$ candidate polluted sequences.}
    \vspace{-2mm}
    \label{fig:method-Tvalue}
     \vspace{-2mm}
\end{figure}

\subsection{Polluted Sequence Screening}

After generating all possible candidate polluted sequences for each $\bm{x}_{u}\in\mathcal{X}$, we need to screen out the polluted sequences that are most influential on enhancing the recommendation of the target item $v^{x}$. To avoid excessive computational overhead, we greedily screen out the most influential polluted sequence for one user each time, and then combine the polluted sequences screened out for all users to form the final attacked training data $\mathcal{X}^{\prime}$. We next concentrate on how to screen out the most influential polluted sequence for each user. 

Toward the goal, we first need to quantify the influence of each polluted sequence on enhancing the recommendation of target item $v^{*}$. To quantify the influence of a polluted sequence $\bm{x}_{u(\delta_{p})}$, the most straightforward way is to compare the recommendation results between the original model and the model obtained by replacing $\bm{x}_{u}$ with $\bm{x}_{u(\delta_{p})}$. However, directly retraining the model could be inefficient. We thus consider utilizing the influence function to estimate the influence with a similar idea but without explicitly retraining. We next first define the influence via the influence function and then present how to calculate it, followed by how to filter the most influential polluted sequences.

\vspace{+5pt}
\subsubsection{Define the Influence of Polluted Sequence on the Target Item.} We first present the basic definition of the utilized influence, and then introduce its detailed expression.

\noindent \textbf{Basic definition.}
For the original model and the model gotten by replacing $\bm{x}_{u}$ with $\bm{x}_{u(\delta_{p})}$, we could represent them with a uniform formulation by adding the loss difference of fitting $\bm{x}_{u}$ and $\bm{x}_{u(\delta)}$ into the original training loss with a weight $\epsilon$ in Equation~\eqref{eq:training-loss} as follows:

\begin{equation}
\begin{split}
\label{params}
    \begin{aligned}
        \hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}}=\mathop{\arg\min}\limits_{\theta} \frac{1}{n}\sum_{u^{\prime}\in\mathcal{U}} L(\bm{x}_{u^{\prime}};\theta) \\ +  \epsilon (L(\bm{x}_{u(\delta p)};\theta)- L(\bm{x}_u;\theta)).
    \end{aligned}
    \end{split}
\end{equation}
The first term corresponds to the training loss on $\mathcal{X}$, identical to Equation~\eqref{eq:training-loss}. The terms $L(\bm{x}_{u(\delta p)},\theta)$ and $L(\bm{x}_u,\theta)$ represent the fitting losses for $\bm{x}_{u(\delta p)}$ and $\bm{x}_{u}$ with the model parameterized by $\theta$, respectively. It is easily verified that: 1) $\hat{\theta}_{\epsilon=0,x_u,x_{u(\delta p)}}$ corresponds to the original model, \ie $\hat{\theta} = \hat{\theta}_{\epsilon=0,x_u,x_{u(\delta p)}}$; and 2) $\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}}$ corresponds to the model gotten by  replacing $\bm{x}_{u}$ with $\bm{x}_{u(\delta_{p})}$. 

To quantify the influence of $\bm{x}_{u}$ on enhancing the recommendation of target item $v^{*}$, we only need to compare the difference between $\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}}$ and  $\hat{\theta}_{\epsilon=0,x_u,x_{u(\delta p)}}$ on recommending the target item $v^{*}$. We formalize the difference with a cross-entropy loss as follows:

\begin{equation}
\begin{split}
     R(\bm{x}_{u(\delta)} \leftarrow \bm{x}_{u}) = L_{atk}(\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}};v^{*})    \\ - L_{atk}(\hat{\theta}_{\epsilon=0,x_u,x_{u(\delta p)}};v^{*}),
\end{split}
\end{equation}
where $R(\bm{x}_{u(\delta)} \leftarrow \bm{x}_{u})$ denotes the difference, and $L_{atk}(\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}};v^{*})$ denotes how likely the model with $\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}}$ would recommend the target item $v^{*}$, which is computed according to the cross-entropy loss, formally,
\begin{equation} 
\label{L_{atk}}
\begin{aligned}
L_{atk}(\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}};v^{*}) = \sum_{u} L_{ce} (f_{\hat{\theta}_{\epsilon=\frac{1}{n},x_u,x_{u(\delta p)}}}(\bm{x}_{u});v^{*}),
\end{aligned}
\end{equation}
where $L_{ce}(\cdot;v^{*})$ denotes the cross-entropy loss regarding the target item $v^{*}$, with lower value denoting a higher probability to recommending $v^{*}$. Then, according to Taylor's series, we have:

\begin{equation}
    \begin{split}
        R(\bm{x}_{u(\delta)} \leftarrow \bm{x}_{u}) &\approx \frac{\partial L_{atk}(\hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}};v^{*})  }{\partial \epsilon} \bigg|_{\epsilon=0} \times \frac{1}{n}\\
        & \propto \frac{\partial L_{atk}(\hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}};v^{*})  }{\partial \epsilon} \bigg|_{\epsilon=0}
    \end{split}.
\end{equation}
This equation means we could define the influence of $\bm{x}_{u(\delta)}$ on promoting the target item $v^{*}$ as:
\begin{equation}
\label{I-atk(noparam)}
    \begin{aligned}
        I_{\epsilon,atk}(x_u,x_{u(\delta p)}) \overset{def}{=} \frac{\partial L_{atk} (\hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}};v^{*})}{\partial \epsilon} \bigg\rvert_{\epsilon=0}
    \end{aligned},
\end{equation}
for which a higher value means a higher influence on enhancing the recommendation of $v^{*}$. We next introduce how to further derive it to make it calculable.



\vspace{+5pt}
\noindent \textbf{Detailed expression.} We have defined the influence of a polluted sequence $\bm{x}_{u(\delta)}$ on enhancing the recommendation of $v^{*}$ based on $\hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}}$ in Equation~\eqref{params}. We next further derive it such that it could be easily calculated according to the model parameters $\hat{\theta}$ trained with the original dataset. According to the Chain rule, we have:
\begin{small}
\begin{equation}
\label{eq:chin-rule}
    \begin{aligned}
        I_{\epsilon,atk}(x_u,x_{u(\delta p)}) & {=} \frac{\partial L_{atk} (\hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}};v^{*})}{\partial \epsilon} \bigg\rvert_{\epsilon=0}\\
        & = \nabla_{\theta} L_{atk} (\hat{\theta}; v^{*}) ^ \top  \frac{\partial \hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}}}{\partial \epsilon} \bigg\rvert_{\epsilon=0}
    \end{aligned},
\end{equation}
\end{small}
where the second term $I_{\epsilon,p}=\frac{\partial \hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}}}{\partial \epsilon} \bigg\rvert_{\epsilon=0}$ is the influence of $\bm{x}_{u}$ on the model parameters. According to the classical results~\cite{DBLP:conf/www/FangG020}, $I_{\epsilon,p}$ can be expressed as follows:


\begin{equation}\small
\begin{split}
\label{I-theta}
\begin{aligned}
    I_{\epsilon,p} & = \frac{\partial \hat{\theta}_{\epsilon,x_u,x_{u(\delta p)}}}{\partial \epsilon} \bigg\rvert_{\epsilon=0}
     = -(H_{\hat{\theta}}+\lambda{I})^{-1} \\ &\quad  *\nabla_{\theta} \big(L(x_{u(\delta p)};\hat{\theta})- L(x_u;\hat{\theta})\big),
    % \\ &\approx -(H_{\theta}+\lambda{I})^{-1}\nabla_{x_u} \nabla_{\theta} L(x_u,\theta))(x_{u(\delta p)})-(x_u).
\end{aligned}
\end{split}
\end{equation}

where $H_{\hat{\theta}} = \frac{1}{n}\sum_{u^{\prime}\in\mathcal{U}} \nabla_{\theta}^2 L(x_{u^{\prime}};\hat{\theta})$ is the Hessian matrix, $L(\cdot)$ denotes the loss defined in Equation~\eqref{eq:training-loss}, $I$ is a identity matrix, and $\lambda$ is a weighting coefficient.  Note that for the original form of the influence function in~\cite{DBLP:conf/icml/KohL17}, there is not a term of $\lambda I$, \ie $\lambda=0$, with assuming that $H_{\hat{\theta}}$  is positive definite. However, the assumption is not usually satisfied for sequential models, we thus follow previous work~\cite{DBLP:journals/corr/abs-2209-05364} to add the term of $\lambda I$, making $H_{\hat{\theta}}+\lambda I$ invertible. 




\textit{{Final expression.}} According to Equation \eqref{I-theta} and Equation~\eqref{eq:chin-rule}, the influence $I_{\epsilon,atk}(x_u, x_{u(\delta p) )})$ could be fully computed with only $\hat{\theta}$ and the defined training loss function $L(\cdot)$ and $L_{atk}(\cdot)$ as follows: 


\begin{equation}\small
\begin{split}
\label{I-atk(param)}
    \begin{aligned}
        I_{\epsilon,atk}(x_u,x_{u(\delta p)}) & = -\nabla_{\theta}L_{atk}(\hat{\theta};v^{*})^T (H_{\hat{\theta}}+\lambda{I})^{-1} \\ &\quad  * \nabla_{\theta}\big(L(x_{u(\delta p)};\hat{\theta})- L(x_u;\hat{\theta})\big)     
    \end{aligned}.
\end{split}
\end{equation}


 
 
 

 \vspace{+5pt}
\subsubsection{Calculate the Influence.}   
Estimating $I_{\epsilon,atk}(x_u,x_{u(\delta p)})$ involves forming and inverting the $H_{\hat{\theta}}+\lambda I$, which could  be computation-costly. 
%Hessian matrix $H_{\hat{\theta}}$ regarding the training loss,
To efficently computing $H_{\theta}$ explicitly, we approximate $H_{\theta}^{-1}$ using the  stochastic estimation proposed in   ~\cite{DBLP:conf/icml/KohL17}. For clarity, let $\Tilde{H} = H_{\hat{\theta}}+\lambda I$, and let $\Tilde{H}_{j}^{-1} = \sum_{i=1}^{j}(I-\Tilde{H}_{j})^{i}$, the first $j$-th terms of the Taylor expansion of $H^{-1}$. And we can re-write $\tilde{H}_{j}^{-1}$ in a recursive form as: $\tilde{H}_{j}^{-1}= I+ (I-\tilde{H}) \tilde{H}_{j-1}^{-1}$. Then it is easily verified that   $\Tilde{H}_{j}^{-1} \rightarrow \Tilde{H}^{-1}$. 

Particularly, at each iteration $j$, we can sample a user $u$, and take $\nabla_{\theta}^{2} L(x_{u};\hat{\theta})$ as an unbiased estimation of the full $\tilde{H}$. After running $J$ interactions, we could approach $\tilde{H}$ with  $\Tilde{H}_{J}^{-1}$. We could run the process multiple times, and take the average of $\Tilde{H}_{J}^{-1}$ as a better estimation for $\tilde{H}$, still denoted as $\tilde{H}_{J}^{-1}$. Finally, we could compute $I_{\epsilon,atk}(x_u,x_{u(\delta p)})$ as follows:

\begin{equation}
\begin{split}
\label{I-atk-compute}
    I_{\epsilon,atk}(x_u,x_{u(\delta p)}) & = -\nabla_{\theta}L_{atk}(\hat{\theta};v^{*})^T \tilde{H}_{J}^{-1} \\ &\quad *\nabla_{\theta}\big(L(x_{u(\delta p)};\hat{\theta}) - L(x_u;\hat{\theta})\big).
\end{split}
\end{equation}




Therefore, to estimate $I_{\epsilon,atk}(x_u,x_{u(\delta p)})$, the stochastic estimation method avoids the explicit calculation of the inverse of the Hessian matrix, which accelerates the calculation of the influence value.




\subsubsection{Filtering}
Finally, for each candidate polluted sequence $\bm{x}_{u(\delta_{p})}$ of the user $u$, we could compute its influence as $I_{\epsilon,atk}(x_u,x_{u(\delta_{p})})$. 
Then, we select the one with the largest absolute value of influence as the final pollution sequence, as shown below:
% Then, we select the one with the highest influence as the final polluted sequence as follows:
$$x_{u}^{\prime} = \bm{x}_{u(\delta_{p^{\prime}})},\quad p^\prime = argmax_{p\in\{1,\dots,m\}} |I_{\epsilon,atk}(x_u, x_{u(\delta_{p})})|.$$
Lastly, the final attack training data $\mathcal{X}^{\prime}$ is constructed by combining all $\bm{x}_{u}^{\prime}$, \ie  $\mathcal{X}^{\prime}=\{\bm{x}_{u}^{\prime}|u\in \mathcal{U}\}$.



\subsection{Constructing the Attack Process}
% Our proposed algorithm can pollute the recommender system by injecting the most influential items to perturb the sequence of users. Ideally, the contamination sequence leads to increased exposure to the target item. To make the attack algorithm clearer, the detailed steps of the attack are described in Algorithm(\ref{alg:INF-atk}).

The INFAttck method aims to manipulate recommender systems by contaminating user interaction sequences to increase exposure to a specific item. To provide a clear understanding of the algorithm, we present Algorithm (\ref{alg:INF-atk}) with detailed attack steps. Firstly, we train the sequential recommender model $f_{\theta}$ on original training data $\mathbf{X}$ to obtain the model parameters $\theta$ (line 2), which are required for the influence computation. Then, we generate the most influential polluted sequence for each user to construct the attacked data $\mathcal{X}^{\prime}$ (lines 3-13). For each user, we cycle $K $times to select the most suitable injection items $ {x_ {u ( delta_ {p})} | p=1,  dots, m } $(lines 4-6), calculate the defined impact of each candidate pollution sequence on the target item (lines 8-10) and ultimately generate the final pollution sequence of user $u $as the sequence with the greatest impact among all candidate pollution sequences (lines 11-12)

\begin{algorithm}[t]
    \caption{INFAttack}
    \LinesNumbered
    \label{alg:INF-atk}
    \KwIn{Original training sequences $\mathcal{X}$, target item $v^{*}$, recommender model $f_{\theta}$, the number of injected items $K$, and the item set $\mathcal{V}$}
    \KwOut{A set of polluted sequences $\mathcal{X}^{\prime}$}
    Initialize $\mathcal{X}^{\prime}=\varnothing$\;
    Train $f_{\theta}$ with $\mathcal{X}$ to obtain $\hat{\theta}$ according to Equation~\eqref{eq:training-loss}\;
    \For{each $x_{u} \in \mathcal{X}$}{
        \While{length of $x_{u(\delta_{p})} $ - length of $x_u < K$}{
            // Step 1: Generate all candidate polluted sequences\;
            Enumerate $m$ possible combinations of $v_{i}^{\prime}$ ($i \leq K$) from $\mathcal{V}$\;
            Inject each $[v_{i}^{\prime}]$ into $\bm{x}_{u}$, obtaining $\{x_{u(\delta_{p})}|p=1,\dots,m\}$\;
            // Step 2: Filter pollution sequences\;
            Compute $I_{\epsilon,atk}(x_u,x_{u(\delta_p)})$ with $\hat{\theta}$ according to Equation~\eqref{I-atk-compute}\;
            \If{max($I_{\epsilon,atk}(x_u,x_{u(\delta_p)})) < 0$}
            {
              \STATE break;
            }              
            \Else
               { Find $p^{\prime} = \text{argmax}_{p} \, |I_{\epsilon,atk}(x_u,x_{u(\delta_p)})|$\;
                $x_{u} = x_{u(\delta_{p})}$\;
                Append $x_{u(\delta_{p^{\prime}})}$ into $\mathcal{X}^{\prime}$\;
               }
            
        }
    }
  Return $\mathcal{X}^{\prime}$
\end{algorithm}


% \begin{algorithm}[t]
%     \caption{INFAttack}
%     \LinesNumbered
%     \label{alg:INF-atk}
%     \KwIn{Original training sequences $\mathcal{X}$, target item $v^{*}$, recommender model $f_{\theta}$, the number of injected items $K$, and the item set $\mathcal{V}$}
%     \KwOut{A set of polluted sequences $\mathcal{X}^{\prime}$}
%     Initialize $\mathcal{X}^{\prime}=\varnothing$\;
%     Train $f_{\theta}$ with $\mathcal{X}$ to obtain $\hat{\theta}$ according to Equation~\eqref{eq:training-loss}\;
%     \For{each $x_{u} \in \mathcal{X}$}{
%     \While{length of $x_{u(\delta_{p})} $-length of $x_u < K$}{
%    // Step 1: Generate all candidate polluted sequence\;
%     Enumerate $m$ possible combinations of $v_{i}^{\prime}(i<=K)$ from $\mathcal{V}$\;
%     Inject each $[v_{i}^{\prime}]$ into $\bm{x}_{u}$, getting $\{x_{u(\delta_{p})}|p=1,\dots,m\}$\;
%     // Step 2:  Filter pollution sequences\;
   
%     Compute  $I_{\epsilon,atk}(x_u,x_{u(\delta_p)})$ with $\hat{\theta}$ according to Equation~\eqref{I-atk-compute}\; 
%     \IF{max($I_{\epsilon,atk}(x_u,x_{u(\delta_p)})$)<0}
% 		\STATE  break;
%     \ELSE
% 		Find $p^{\prime} = argmax_{p} \, I_{\epsilon,atk}(x_u,x_{u(\delta_p)})$\;
%         $x_{u}=x_{u(\delta_{p})}$;
%         Append $x_{u(\delta_{p^{\prime}})}$ into $\mathcal{X}^{\prime}$\;
%     \ENDIF
    
%     }   
%     } 
%     Return $\mathcal{X}^{\prime}$
 
% \end{algorithm}  




